ALMA detections of circumstellar disks in the giant Hii region M17. Probing the intermediate- to high-mass pre-main-sequence population

Our current understanding is that intermediate- to high-mass stars form in a way similar to low-mass stars, that is, through disk accretion. However, the physical conditions that play a role in disk formation, evolution, and the possibility of (sub)stellar companion formation, are significantly different. We search for the mm counterparts of four intermediate- to high-mass (4-10 Solar mass) young stellar objects (YSOs) in the giant Hii region M17 at a distance of 1.7 kpc. These objects expose their photospheric spectrum such that their location on the pre-main-sequence (PMS) is well established. They have a circumstellar disk that is likely remnant of the formation process. With ALMA we have detected, for the first time, these four YSOs in M17, in Band 6 and 7, as well as four other serendipitous objects. Besides the flux measurements, the source size and spectral index provide important constraints on the physical mechanism(s) producing the observed emission. We apply different models to estimate the dust and gas mass contained in the disks. All our detections are spatially unresolved, constraining the source size to <120 au, and have a spectral index in the range 0.5-2.7. The derived (upper limits on the) disk dust masses are on the order of a few Earth masses and estimations of the upper limits on the gas mass vary between $10^{-5}$ and $10^{-3}$ Solar mass. In two objects (B331 and B268) free-free emission indicates the presence of ionized material around the star. The four serendipitous detections are likely (low-mass) YSOs. We compare the derived disk masses of our M17 targets to those obtained for YSOs in low-mass star-forming regions (SFRs) and Herbig stars, as a function of stellar mass, age, luminosity, and outer disk radius. The M17 sample, though small, is both the most massive and the youngest sample, yet has the lowest mean disk mass.

==> tables/CO_detection_rates.tex <==
\newcolumntype{C}{>{\centering\arraybackslash}m{0.056\linewidth}}
\newcolumntype{D}{>{\centering\arraybackslash}m{0.09\linewidth}}
\newcolumntype{O}{>{\centering\arraybackslash}m{0.165\linewidth}}
\newcolumntype{R}{>{\centering\arraybackslash}m{0.195\linewidth}}

\begin{table*}[ht!]
\footnotesize
\centering
\caption{Detection rates of CO \first\, overtone bandhead emission (CO emission) in YSOs of different masses and stages of formation. }  
\begin{minipage}{\hsize}
\centering
\renewcommand{\arraystretch}{1.4}
% \setlength{\tabcolsep}{3pt}
\begin{tabularx}{\linewidth}{D|O|C|C|X|R}
\toprule
Mass\footnote{The mass categories refer to expected ZAMS masses of approximately $\lesssim 2$ \msun (low), $2-8$ \msun (intermediate) and $\gtrsim 8$ \msun (high). Since mass estimates are not always available or derived in the same way the numbers are approximate.} & Object type & Detection rate & Sample size  & Comments & Reference \\
\midrule
Low & Class 0 & 67\% & 6 & &\cite{laos2021} \\
Low & Class I & 15\% & 52 & &\cite{doppmann2005} \\
Low & Class I & 22\% & 110 & &\cite{connelley2010} \\
Low  & T Tauri &  0\% & 100 & Sample from Lupus region. Authors find 3 cl TTS with CO emission in literature. &\cite{koutoulaki2019}   \\
Low to intermediate & Variable, embedded (EXors, FUors, MNors) & 38\% & 28 &  60\% among objects identified as eruptive YSOs undergoing an episode of accretion. & \cite{contreraspena2017}  \\
Intermediate & Herbig AeBe & 5-21\% & 36 & &\cite{ishii2001} \\
Intermediate & Herbig AeBe & 7\% & 91 & Strong preference for higher mass objects. & \cite{ilee2014}   \\
High & MYSO & 17\% & 195  & Red MSX Source (RMS) survey; low resolution spectroscopy. & \cite{cooper2013}\\
High & MYSO (without \Hii\,region) & 34\% & 36  & Subsample RMS, selected to be luminous and radio quiet; intermediate resolution spectroscopy. & \cite{pomohaci2017}\\
High & MYSO (with and without \Hii\,region) & 18\% & 11  & Sources associated with a disk (candidate) in sub-mm/radio and with a bright NIR counterpart. & \cite{hsieh2021}\\
\midrule
Intermediate to high & PMS stars in M17 & 63-83\% & 6-8 & Sample from which the objects in this study were taken.  & RT17 \\
\bottomrule
% \vspace{-15pt}
\end{tabularx}
\end{minipage}
\label{tab:CO_detection_rates}
\normalsize
\end{table*}

==> tables/band7.tex <==
\begin{table*}[ht!]
\footnotesize
\centering
\caption{}       % title of Table
\begin{minipage}{0.9\hsize}
\centering
\renewcommand{\arraystretch}{1.4}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{ccccccccc}
\hline
Obj & uvrange & rms & RA & RA\_e & dec & dec\_e & peak flux & err (mJy) \\
& & (mJy) & & (mas) & & (mas) & (mJy) & (mJy) \\
\hline
B275 & all & 0.0575 & $18:20:25.0276$ & 3 & $-16.10.26.146$ & 2 & $0.573$ & $  0.045$ \\
B275a & $\rm separation$ & 5.0'' & $18:20:25.1346$ & 3 & $-16.10.30.889$ & 2 & $0.448$ & $  0.045$ \\
B331 & $> 500 k\lambda$ & 0.0831 & $18:20:21.6372$ & $<1$ & $-16.11.17.947$ & $<1$ & $1.846$ & $  0.049$ \\
B331a & $\rm separation$ & 1.38'' & $18:20:21.6061$ & 2 & $-16.11.16.637$ & 1 & $0.720$ & $  0.040$ \\
B331b & $\rm separation$ & 5.2'' & $18:20:21.5805$ & 1 & $-16.11.23.015$ & $<1$ & $1.117$ & $  0.035$ \\
B331c & $\rm separation$ & 6.6'' & $18:20:21.9234$ & 5 & $-16.11.12.741$ & 3 & $0.441$ & $  0.060$ \\
B243 & all & 0.0556 & $18:20:26.5599$ & 2 & $-16.10.03.339$ & 1 & $0.476$ & $  0.028$ \\
B243a & $\rm see~band~6$ & & $18:20:26.3455$ & 7 & $-16.10.06.749$ & 1 & $0.257$ & $  0.031$ \\
B268 & all & 0.0577 & - & - & - & - & $0.138$ & $  0.013$ \\
\hline
\end{tabular}



\centering
% \tablefoot{}
\end{minipage}
\label{tab:band7}
\normalsize

\end{table*}

==> tables/positions_and_fluxes_band6.tex <==
\begin{table*}[ht!]
\footnotesize
\centering
\caption{}       % title of Table
\begin{minipage}{0.9\hsize}
\centering
\renewcommand{\arraystretch}{1.4}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{ccccccccccc}
\hline
Obj & uvrange & rms & RA & err (mas) & dec & err (mas) & peak flux & err (mJy) & VLA flux \\
& & (mJy) & & & & & (mJy) & (mJy) & (mJy) \\
\hline
B275 & $>50k\lambda$ & 0.0232 & $18:20:25.0271$ & 3 & $-16.10.26.140$ & 1 & 0.279 & 0.016 & $<0.025$ \\
B275a & $\rm see~band~7$ & & $18:20:25.1350$ & 4 & $-16.10.30.889$ & 2 & 0.250 & 0.021 & $<0.025$ \\
B331 & $> 500 k\lambda$ & 0.0395 & $18:20:21.6371$ & 0.6 & $-16.11.17.944$ & 0.3 & 1.485 & 0.029 & $0.286 \pm0.022$ \\
B331a & $\rm see~band~7$ & & $18:20:21.6063$ & 2 & $-16.11.16.639$ & 1 & 0.280 & 0.021 & $<0.025$ \\
B331b & $\rm see~band~7$ & & $18:20:21.5801$ & 2 & $-16.11.23.012$ & 1 & 0.410 & 0.033 & $<0.025$ \\
B331c & $\rm see~band~7$ & & - & - & - & - & <0.119 & - & $<0.025$ \\
B243 & $>50k\lambda$ & 0.0218 & $18:20:26.5596$ & 6 & $-16.10.03.339$ & 3 & 0.158 & 0.018 & $<0.025$ \\
B243a & $\rm separation$ & 4.6'' & $18:20:26.3456$ & 3 & $-16.10.06.748$ & 1 & 0.201 & 0.014 & $<0.025$ \\
B268 & $>50k\lambda$, $\rm uvt~0.08''$ & 0.0313 & $18:20:25.2872$ & 9 & $-16.10.18.497$ & 6 & 0.138 & 0.013 & $<0.025$ \\
\hline
\end{tabular}






\centering
% \tablefoot{}
\end{minipage}
\label{tab:positions_and_fluxes_band6}
\normalsize

\end{table*}
